Performance Benchmarking and Optimizing Hyperledger Fabric Blockchain Platform

The rise in popularity of permissioned blockchain platforms in recent time is significant. Hyperledger Fabric is one such permissioned blockchain platform and one of the Hyperledger projects hosted by the Linux Foundation. The Fabric comprises various components such as smart-contracts, endorsers, committers, validators, and orderers. As the performance of blockchain platform is a major concern for enterprise applications, in this work, we perform a comprehensive empirical study to characterize the performance of Hyperledger Fabric and identify potential performance bottlenecks to gain a better understanding of the system. We follow a two-phased approach. In the first phase, our goal is to understand the impact of various configuration parameters such as block size, endorsement policy, channels, resource allocation, state database choice on the transaction throughput & latency to provide various guidelines on configuring these parameters. In addition, we also aim to identify performance bottlenecks and hotspots. We observed that (1) endorsement policy verification, (2) sequential policy validation of transactions in a block, and (3) state validation and commit (with CouchDB) were the three major bottlenecks. In the second phase, we focus on optimizing Hyperledger Fabric v1.0 based on our observations. We introduced and studied various simple optimizations such as aggressive caching for endorsement policy verification in the cryptography component (3x improvement in the performance) and parallelizing endorsement policy verification (7x improvement). Further, we enhanced and measured the effect of an existing bulk read/write optimization for CouchDB during state validation & commit phase (2.5x improvement). By combining all three optimizations1, we improved the overall throughput by 16x (i.e., from 140 tps to 2250 tps).

==> tex/resources.tex <==
%IMPACT OF RESOURCES 
\input{tex/tables/cpu.tex}
\begin{figure}
%  \vspace{-.2cm}
    \begin{center}
     \includegraphics[scale=0.4]{graphs/cpu-throughput.pdf}
    %\hrule width \hsize height .33pt
     %\vspace{-.4cm}
     \caption{Impact of number of vCPU cores on throughput and latency when the number of
     channel was 4 and transaction arrival rate was 350.}
   \label{fig:compress-comp}
 \end{center}
  %\vspace{-.7cm}
\end{figure}




